EDF-VD Scheduling of Mixed-Criticality Systems with Degraded Quality Guarantees

This paper studies real-time scheduling of mixed-criticality systems where low-criticality tasks are still guaranteed some service in the high-criticality mode, with reduced execution budgets. First, we present a utilization-based schedulability test for such systems under EDF-VD scheduling. Second, we quantify the suboptimality of EDF-VD (with our test condition) in terms of speedup factors. In general, the speedup factor is a function with respect to the ratio between the amount of resource required by different types of tasks in different criticality modes, and reaches 4/3 in the worst case. Furthermore, we show that the proposed utilization-based schedulability test and speedup factor results apply to the elastic mixed-criticality model as well. Experiments show effectiveness of our proposed method and confirm the theoretical suboptimality results.

==> tuning.tex <==
\section{Enhancement for IMC}
\label{section:tuning}
% In some cases, the given task set might not pass the schedulability test. 
% In the regular MC system, the system tends to at least ensure the schedulability of all \hi tasks if the system switches to the \hi mode. 
% Hence, if the given IMC task set does not satisfy the test, 
% the IMC task set has to drop off some \lo tasks in order to ensure the schedulability of all \hi tasks as the regular MC model ensures. 
% Dropping off \lo tasks can be done by setting $C_i^{HI}$ equal to 0. 
% There can be several different metrics to drop off tasks, e.g., drop off the least important task first or drop off as few tasks as possible. 
% This is mainly determined by the system designers. 
% As long as a drop-off strategy is given, the strategy finds some \lo tasks as drop-off candidates 
% and discards them one by one to ensure the schedulability of the \hi tasks while keeping some \lo tasks, if possible.
%  
% On the other hand, if the given task set passes the schedulability test, 
% there might be some space for \lo tasks to increase their $C_i^{HI}$. 
% As we explained in Section \ref{section:background}, the output quality of a \lo task improves over its execution time, 
% so increasing $C_i^{HI}$ is able to improve its output quality.  
% Similar to drop-off strategies, the system can have different selection strategies to enhance the quality, 
% e.g., important task first, total quality of the system, etc. 
% However, although the system designer can determine the metric for the improvement, 
% it has to be determined how to distribute the slack among each \lo tasks so 
% that the benefit according to the metric is maximized. 
% Hence, in the next section, we propose a linear programming (LP) approach to solve this problem, 
% where the LP approach can be used for different metrics. 
Section \ref{section:sufficientTest} and \ref{section:speed} provide the theoretical foundation for 
the IMC model. In this section, we propose two enhancement techniques for the IMC model. 
One enhancement is to improve the output quality of \lo tasks if the task set initially satisfies the 
sufficient test given in Theorem \ref{theorem:overall}. Another enhancement is to improve the schedulability of the whole system if the initial task set fails the proposed test.

Priori to introduce the enhancements, we first extend our model by integrating a new notion \textit{importance} to \lo tasks. 
Fleming and Burns in \cite{fleming2014incorporating} have introduced the notion of \textit{importance} to \lo tasks, where the \lo tasks are dropped off sequentially based on the \textit{importance} when the \hi tasks overrun. 
In the IMC model, we let the \textit{importance} notion define which \lo tasks are preferred to obtain the better quality in the \hi mode. This can be decided by the system designers. 
We use $w_i$ to denote the \textit{importance} for \lo task $\tau_i$, where the large value of $w_i$ means \lo task $\tau_i$ is more \textit{important} . 

Moreover, we define a quality ratio for each \lo task. Let $Q_i$ denote the quality ratio for \lo task $\tau_i$.
\begin{definition}
\label{definition:quality}
 A quality ratio $Q_i$ of \lo task $\tau_i$ is defined as
 \begin{equation}
  \label{definition:quality_ratio}
  Q_i = \frac{C_i^{HCM}}{C_i^{LCH}}
 \end{equation}
 where $Q_i = 0$ or $ M_i \le Q_i\le 1$ where $M_i$ denotes the mandatory quality ratio.
\end{definition}
Here, the mandatory quality ratio means the smallest quality ratio \lo task $\tau_i$ needs to ensure 
such that the task can produce a useful result. This concept is similar to the mandatory execution time 
in the original \textit{imprecise model}  \cite{Liu1991}\cite{Liu1994}. When $Q_i=0$, it is dropped off after the system overruns, i.e., no execution in the \hi mode. If $\tau_i$ executes in the \hi mode, 
it ensures to satisfy $ M_i \le Q_i\le 1$.

The feature of \lo tasks in the IMC model indicates that the longer the task executes, 
the better quality the task produces. 
Thus, we use $Q_i$ to quantify the quality loss of task $\tau_i$ 
when the system switches to the \hi mode.  
% $Q_i$ serves  as the metric to justify the quality of one \lo task. 
To measure the quality of all \lo tasks we need to take into account the \textit{importance} of \lo tasks. 
We give the following definition, 
\begin{definition}
\label{definition:total}
 The weighted total quality (WTQ) of all \lo tasks in an IMC task set $\gamma$ is defined as,
\begin{equation}
 Q = \sum\limits_{\tau_i \in \gamma_{LCT}}Q_iw_i
\end{equation}
where $\gamma_{LCT}$ is all \lo tasks.
\end{definition}
With the definitions above, we will introduce the two enhancements for the IMC model.

% 
% The schedulability test presented in Section \ref{section:sufficientTest} can be used to check the schedulability of a given task set. 
% % A given task set can be identified either schedulable or unschedulable by the schedulability test. 
% For a schedulable task set, since \lo tasks trade off their quality for their schedulability, in this section we explore its design space to reduce the quality loss, 
% i.e., increase $C_i^{HI}$ of \lo tasks. 
% Then, for a unschedulable task set, we discuss how to drop off \lo tasks to improve the system schedulability. 
% In the IMC, \lo tasks trade off their quality for their schedulability after the system switches to the \hi mode. 
% Hence, in order to reduce the quality loss, 
% given a schedulable task set, we propose an approach to optimize $C_i^{HI}$ of \lo tasks to maximize their output quality.  
% 
% In this section, given a task set which can ensure the schedulability test in Section \ref{section:sufficientTest}, we propose an approach to explore the slack left to further 
% increase $C_i^{HI}$ of \lo tasks, i.e., improve the output quality of \lo tasks. 
 
% Then, it is important to know what is the execution budget for \lo tasks such that the system maximizes the benefits that \lo tasks can obtain to 
% improve their quality 
 
\subsection{Improving Output Quality of Low Criticality Tasks}
\label{tune:improve}
In this subsection, we propose an integer linear programming (ILP) based approach to optimally maximize the output quality of \lo tasks 
if the IMC task set with their initial settings can satisfy the proposed sufficient test. 
\textit{WTQ} given in Definition \ref{definition:total} provides a good metric to the optimization problem, so we in this scenario aim to maximize \textit{WTQ} of \lo tasks. 
% The objective function can be written as follows:
% \begin{equation}
%  \label{lp:objective}
%  \text{maximize}\quad Q
% \end{equation}
 
% \lo tasks in a system can be distinguished with the different degree of importance. 
% Thus, we use a weighted coefficient to denote the importance of a \lo task. 
% Let variable $w_i$ denote the weighted coefficient for \lo task $\tau_i$, 
% where the larger value indicates the higher importance or preference.

Each \lo task is given $C_i^{HCM}$ at the beginning and in this case we consider it as the initial WCET setting for the \hi mode.
 Let $I_i$ represent the extra execution budget 
which \lo task $\tau_i$ can receive in the \hi mode. 
Here, we can take $I_i$ as the optimization variable and build up constraints for $I_i$. 
As we know, \lo tasks can be either dropped off or executed at least the mandatory time to ensure a 
useful result. 
Therefore, we can have two constraints for $I_i$: 1) the initial $C_i^{HCM}$ equals to 0, i.e., \lo task $\tau_i$ is planed to be dropped off;
2) the initial $C_i^{HCM}$ is greater than 0, i.e., \lo task $\tau_i$ has execution budgets in the \hi mode.
For case 1, we have the following constraint for $I_i$,
\begin{equation}
 \label{lp:case_1}
 C_i^{M}\le I_i \le C_i^{LCM}
\end{equation}
where $C_i^{M}$ is the smallest WCET for which \lo task $\tau_i$ should execute to ensure a useful result.
Constraint (\ref{lp:case_1}) guarantees that $I_i$ will receive more than its mandatory execution to satisfy the output quality. 
On the other hand, if $\tau_i$ already has execution budgets in the \hi mode, 
we have the following constraint,
\begin{equation}
 \label{lp:case_2}
 0 \le I_i \le (C_i^{LCM} - C_i^{HCM})
\end{equation}
 In this case, since $\tau_i$ is already assigned a certain execution time in the \hi mode, the selection range of $I_i$ can be bound by $[0, (C_i^{LCM} - C_i^{HCM})]$.

Constraint (\ref{lp:case_1}) and (\ref{lp:case_2}) bound each \lo task, so we need to construct the bound for all \lo tasks. 
We build up the constraint for all \lo tasks via Theorem \ref{theorem:high_crit}. 
Theorem \ref{theorem:high_crit} ensures the schedulability of the IMC mode in the \hi mode.  
If let $U_{LCT}^{I}=\sum_{\forall \tau_i \in \gamma_{LCT}}\frac{I_i}{T_i}$ denote the total increased utilization  which all \lo tasks can have in the \hi mode, then we can have the following:
\begin{equation}
 \begin{split}
  & x\ull + (1-x)(\ulh +U_{LCT}^I )+ \uhh \le 1\\
  & \iff (1-x) U_{LCT}^I \le 1 -x\ull - (1-x)\ulh - \uhh 
 \end{split}
\end{equation}
 Since $(1-x) > 0$, we obtain the following constraint for all \lo tasks,
 \begin{equation}
\label{lp:alltasks}
 U_{LCT}^I \le \frac{1}{(1-x)} -\frac{x}{(1-x)}\ull - \ulh - \frac{\uhh}{1-x} 
 \end{equation}

Now, all constraints of the optimization problem are given above in constraint (\ref{lp:case_1}),(\ref{lp:case_2}), and (\ref{lp:alltasks}). The objective function of our problem is as follows,
\begin{equation}
 \text{maximize: } \sum_{\forall \tau_i \in \gamma_{LCT}} \frac{C_i^{HCM} +I_i}{C_i^{LCM}}w_i
\end{equation}
 Since $\frac{C_i^{HCM}}{C_i^{LCM}}w_i$ is a constant, we obtain a simplified objective function,
\begin{equation}
\label{lp:objective}
 \text{maximize: } \sum_{\forall \tau_i \in \gamma_{LCT}} \frac{I_i}{C_i^{LCM}}w_i
\end{equation}
Then, optimizing the output quality for \lo tasks in the IMC model is formulated as the following ILP problem:
\begin{equation}
 \label{equation:lp}
 \begin{split}
   & \text{maximize: }  \sum_{\forall \tau_i \in \gamma_{LCT}} \frac{w_i}{C_i^{LCM}}I_i \\
  & U_{LCT}^I \le \frac{1}{(1-x)} -\frac{x}{(1-x)}\ull - \ulh - \frac{\uhh}{1-x}  \\
  & C_i^{M}\le I_i \le C_i^{LCM}, \quad \forall \tau_i \in \gamma_{LCT}, C_i^{HCM} = 0 \\
  & 0 \le I_i \le (C_i^{LCM} - C_i^{HCM}), \quad \forall \tau_i \in \gamma_{LCT}, C_i^{HCM} \neq 0
 \end{split}
\end{equation}

By solving Eq. (\ref{equation:lp}), we can obtain an optimized WCET setting for all \lo tasks in the \hi 
mode under the proposed sufficient test. 
% 
% Therefore, instead of optimizing variable $I_i$, we take $u_i^{ex}=\frac{I_i}{T_i}$ as the optimization 
% variable. 
% In order to formulate the problem as a LP, instead of optimizing $I_i$, we let $u_i^{ex}$ equal to $\frac{I_i}{T_i}$
% We can set up constraints for our optimization problem. 
% 
% 
% If it were dropped off, \lo task $\tau_i$ has the following constraint,
% \begin{equation}
%  \label{lp:task_1}
%  u_i^{M}\le u_i^{ex} \le u_i^{LCM}
% \end{equation}
%  
% Moreover, we use $u_i^{ex}$
% With the consideration of weighted coefficient $w_i$, the total quality of all \lo tasks in an IMC task set is given as follows: 
% \begin{equation}
%  \label{equation:total_quality}
%  E = \sum_{\forall L_i = LO} \frac{C_i^{HI} + I_i}{C_i^{LO}}w_i
% \end{equation}
% where variable $I_i$ denote the time budgets which \lo task $\tau_i$ obtains to increase $C_i^{HI}$. 
% Since $\frac{C_i^{HI}}{C_i^{LO}}w_i$ is a constant and we want to maximize the value of Eq. (\ref{equation:total_quality}), 
% the objective function of our optimization problem can be defined as follows:
% \[\text{max} \sum_{\forall L_i = LO} \frac{I_i}{C_i^{LO}}w_i\]
% Let variable $S$ denote, 
% \[S = 1 - x\ull -(1-x)\ulh - \uhh\]
% We see that the optimization space is constrained by inequality (\ref{equation:edfvd_upper}).  
% Hence, the optimization space must be smaller than or equal to $S$. 
% Then, the following inequality builds up one constraint for our optimization problem.
% \begin{equation}
%  \sum_{\forall L_i = LO} \frac{I_i}{T_i} \le S
% \end{equation}
% The lower bound and upper bound of $I_i$ are formulated as follows:
% {\small
% \begin{equation}
% \label{ilp:non_zero}
%  0 \le \frac{I_i}{T_i} \le u_i(LO)-u_i(HI), \quad \forall L_i = LO, C_i^{HI} \neq 0
% \end{equation}
% \begin{equation}
% \label{ilp:zero}
%  u_i(HI) \le \frac{I_i}{T_i} \le u_i(LO), \quad \forall L_i = LO, C_i^{HI} = 0
% \end{equation}}
% Constraint (\ref{ilp:non_zero}) is used to bound the execution of the \lo task that initially has execution budgets in the \hi mode, 
% whereas constraint (\ref{ilp:zero}) tends to bound the execution of the \lo task which initially was considered to be dropped off completely. 
% For this case, the lower bound needs to guarantee an useful output of the \lo task, if it has some execution budgets assigned after optimization.   
% Let $u_i^{ex}$ denote $\frac{I_i}{T_i}$. The objective function can be rewritten as follows:
% \[ \text{max} \sum_{\forall L_i = LO} \frac{u_i^{ex}}{u_i(LO)}\cdot w_i \]
% Then, optimizing the quality of \lo tasks in an IMC task set is formulated as the following linear programing (LP) problem:
% % Since $I_i$ must be an integer number, the optimization problem becomes an integer linear programing (ILP) problem. 
% {\small
% \begin{equation}
%  \label{equation:lp}
%  \begin{split}
%    \text{max} & \sum_{\forall L_i = LO} \frac{u_i^{ex}}{u_i(LO)}\cdot w_i \\
%   & \sum_{\forall L_i = LO} u_i^{ex} \le 1 - x\ull -(1-x)\ulh - \uhh \\
%   & 0 \le u_i^{ex} \le u_i(LO)-u_i(HI), \quad \forall L_i = LO, C_i^{HI} \neq 0 \\
%   & u_i(HI) \le u_i^{ex} \le u_i(LO), \quad \forall L_i = LO, C_i^{HI} = 0
%  \end{split}
% \end{equation}}
% 
% As can be seen, if $I_i$ is the optimization variable, the problem can be solved as an integer linear programing (ILP) problem. 
% However ILP is known to be intractable \cite{Papadimitriou1981}, whereas LP can be solved in polynomial time \cite{Karmarkar1984}. 
% Moreover, using LP to approximate ILP has been used efficiently in previous research \cite{Baruah2004}, 
% so we use LP to deal with the intractability of ILP. 
% The solution from Eq. (\ref{equation:lp}) gives $u_i^{ex}$, and we increase $C_i^{HI}$ of \lo task $\tau_i$ by using the following equation:
% \begin{equation}
%  \label{equation:extra}
%  C_i^{HI} = C_i^{HI} +  \lfloor T_i\cdot u_i^{ex}\rfloor
% \end{equation} 
% By giving different values to $w_i$, the designers can achieve different objectives. 
% For example, if some \lo tasks are favored to have good quality, their weighted coefficients can be set to a larger value. 
% On the other hand, if all \lo tasks are treated equally, all weighted coefficients can be set to the same value. 

\subsection{Dropping off low criticality tasks}
\label{tunning:drop}
The preceding section introduces an approach to improve the output quality of \lo tasks in the IMC model when the tasks can initially satisfy the proposed sufficient test. 
However, it may happen that the initial task setting cannot satisfy the proposed sufficient test. 
% Theorem \ref{theorem:overall} provides a schedulability test for a given task set. 
% In some cases the given task set cannot pass this sufficient test. 
In such cases,   
% If a given task set can not pass the schedulability test given in Theorem \ref{theorem:overall}, 
we can drop off some \lo tasks when the system switches to the \hi mode so that 
we ensure the schedulability of the whole system. 

Although the initial task setting which is usually specified by the system designers fails to pass the 
sufficient test, we may still find some slack in the \hi mode for the \lo tasks to execute. 
Therefore, based on the introduced metric \textit{WTQ} we propose an approach to 
improve the schedulability of the IMC model while maximizing \textit{WTQ} (see in Definition \ref{definition:total}) for all \lo tasks.
%  when the initial task setting cannot satisfy the proposed 
% sufficient test. 

Let $Q_i^{w}=Q_iw_i$ denote the quality ratio of \lo task $\tau_i$ with the consideration of the \textit{importance.}
% \begin{equation}
%  \label{equation:quality_importance}
%  Q_i^{w}=\frac{C_i^{HCM}}{C_i^{LCM}}w_i = \frac{\frac{C_i^{HCM}}{T_i}}{\frac{C_i^{LCM}}{T_i}}w_i = \frac
% {u_i^{HCM}}{u_i^{LCM}}w_i
% \end{equation}
We use $Q_i^w$ as the metric to select the drop-off candidate from the \lo tasks 
% which have execution budget in the \hi mode 
and then drop the selected \lo tasks one by one until the task set satisfies the proposed sufficient test.  

% The dropping order has been studied in \cite{fleming2014incorporating} by taking into account the 
% importance of \lo tasks.
Algorithm \ref{algorithm:drop} presents the pseudo-code to drop off \lo tasks in case an unschedulable task set is found. The input is a task set $\gamma$. The algorithm uses Theorem \ref{theorem:overall} to check the schedulability of task set $\gamma$. If task set $\gamma$ cannot pass the test, 
the \lo task with the smallest $Q_i^{w}$ is dropped off (Line 5 and 6). The algorithm terminates when all \lo tasks have been dropped off but the task set still can not pass the schedulability test (Line 3 and 4), or the task set becomes schedulable.  
\begin{algorithm}
 \small
 \caption{Drop off \lo tasks}
  \label{algorithm:drop}
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
 \Input{ IMC task set $\gamma$}
 \Output{ the schedulability of task set $\gamma$ }
%   $x = \frac{\uhl}{1 - \ull}$
% 
%   $D_i = x\cdot T_i, \quad \{\forall \tau_i \in \gamma| L_i = HC\}$

  \While{Theorem \ref{theorem:overall} fails}{

  $\Gamma^{LC} \leftarrow \{\tau_i| L_i = LCT \text{ and } C_i^{HCM} \ne 0\}$
  
%   Sort $\Gamma^{LC}$ in order of increasing $Q_i^{w}$

 \If{$\Gamma^{LC} = \emptyset $}{
      \Return Unschedulable
}
    $\tau_t \leftarrow \argmin\limits_{\tau_i \in \Gamma^{LC}}(Q_i^w)$ 

    $C_t^{HCM}  \gets 0$
    
  }
 \Return Schedulable
\end{algorithm}

The objective of  Algorithm \ref{algorithm:drop} is to ensure the schedulability of the system while maximizing \textit{WTQ} of \lo tasks. 
There can be other different metrics to drop off tasks, e.g., drop off as few tasks as possible. 
This should be determined by the system designers. 
With the proposed enhancement techniques, the system designer can simply specify the mandatory execution time as the \hi-mode WCET for \lo tasks. 
Then, based on whether the task set with the initial WCET settings can pass the proposed sufficient test, the proposed enhancement approaches can be applied to 
improve either the \textit{WTQ} or the schedulability of the system.  
% As long as a drop-off strategy is confirmed, the strategy finds some \lo tasks as drop-off candidates 
% and discards them one by one to ensure the schedulability of the \hi tasks while keeping some \lo tasks, if possible.

% \subsection{The Proposed Algorithm}
% In this section, we present an integrated algorithm in which the proposed sufficient test is used to ensure the schedulability of the IMC system by dropping off some \lo tasks
% or to improve the output quality of \lo tasks by increasing $C_i^{HI}$ of \lo tasks .
% Algorithm \ref{algorithm:tune} gives the pseudo code. 
% The inputs of the algorithm are an IMC task set $\gamma$ and the deadline scale factor $x$, and the output is task set $\gamma$ with new $C_i^{HI}$. 
% First, the algorithm computes $S$ at Line 1. 
% If $S = 0$, the original $\gamma$ is returned without any change at Line 3.
% If $S < 0$, this means that $\gamma$ is not schedulable according to the sufficient test in Theorem \ref{theorem:high_crit}. 
% Thus, from Line 5 to Line 12, the algorithm changes $C_i^{HI}$ of some \lo task to drop off those tasks. 
% In this procedure, a function \textsf{FindTask} is used to find one task according to a given 
% task selection strategy. 
% The algorithm drops off the task given by function \textsf{FindTask} (at Line 11). 
% As long as $S >= 0$, it stops and returns $\gamma$ with the new $C_i^{HI}$ for \lo tasks. 
% However, if $\forall L_i = LO, \quad C_i^{HI} = 0$ and $S > 0$, 
% the task set $\gamma$ is not schedulable even with dropping off all \lo tasks. 
% Hence, the algorithms returns a failure at Line 8. 
% On the other hand, from Line 13 to Line 16, if $S<0$, the algorithm strives to increase $C_i^{HI}$ of the \lo tasks in $\gamma$. 
% At Line 14, function \textsf{LPsolver} solves the LP problem as described in Eq. (\ref{equation:lp}).
% Then, it changes $C_i^{HI}$ of \lo tasks according to the LP solution and Eq. (\ref{equation:extra}). 
% Finally Algorithm \ref{algorithm:tune} returns $\gamma$ with the new $C_i^{HI}$ for \lo tasks in $\gamma$ at Line 16.
% 

% \begin{algorithm}[!t]
%  \small
%  \caption{Enhancement}
%  \label{algorithm:tune}
%   \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
%  \Input{ IMC task set $\gamma$ and $x$}
%  \Output{ $\gamma$ with tuned mandatory executions}
% % \If{The condition in Theorem \ref{theorem:overall} is not ensured}{
% %  \Return unschedulable
% % }
% 
%  $S = 1 - x\ull -(1-x)\ulh - \uhh$;
% 
%  \If{$S = 0$}
% {\Return $\gamma$;}
% 
%  $\gamma^{LO}\leftarrow \tau_i, \quad \forall L_i=LO$;
% 
%  \If{$S < 0 $}{
%  \While{$S < 0$}{
%   \If{$\gamma^{LO} == \emptyset$}{ \Return unschedulable;}
%   $\tau_t\leftarrow$FindTask($\gamma^{LO}$);
% 
%   $\gamma^{LO} \leftarrow \gamma^{LO} - \tau_t$;
% 
%   $C_t^{HI} = 0$, update $\gamma$ and compute a new $S$;
% 
%   }
%   \Return $\gamma$;}
%   
% \If{$S > 0$}{
%  $u_i^{ex}\leftarrow$ LPsolver($\gamma$), $\forall L_i = LO$;
% 
%  $C_i^{HI} = C_i^{HI} + \lfloor T_i\cdot u_i^{ex}\rfloor, \quad \forall L_i = LO$;
% 
%  Update $\gamma$ and \Return $\gamma$;
% }
% \end{algorithm}
